MESH -- Understanding Videos Like Human: Measuring Hallucinations in Large Video Models

Large Video Models (LVMs) build on the semantic capabilities of Large Language Models (LLMs) and vision modules by integrating temporal information to better understand dynamic video content. Despite their progress, LVMs are prone to hallucinations-producing inaccurate or irrelevant descriptions. Current benchmarks for video hallucination depend heavily on manual categorization of video content, neglecting the perception-based processes through which humans naturally interpret videos. We introduce MESH, a benchmark designed to evaluate hallucinations in LVMs systematically. MESH uses a Question-Answering framework with binary and multi-choice formats incorporating target and trap instances. It follows a bottom-up approach, evaluating basic objects, coarse-to-fine subject features, and subject-action pairs, aligning with human video understanding. We demonstrate that MESH offers an effective and comprehensive approach for identifying hallucinations in videos. Our evaluations show that while LVMs excel at recognizing basic objects and features, their susceptibility to hallucinations increases markedly when handling fine details or aligning multiple actions involving various subjects in longer videos.

==> content/ack.tex <==
\begin{acks}
% \acmo{To Robert, for the bagels and explaining CMYK and color spaces.}
\acmo{
Garry YANG, Zizhe Chen, Man Hong Wong are partially supported by RGC Young Collaborative Research Grant No. C2005-24Y.}
\end{acks}

==> tables/stage-table.tex <==
% \begin{table*}[h]
% \centering
% \scriptsize
% \caption{Evaluation results on simple and multi-choice event hallucination questions.}
% \label{tb:combined_event_hallucination}
% \begin{tabular}{lcccccccccccc}
% \toprule
% \textbf{LVLM} & \multicolumn{6}{c}{\textbf{Simple Task}} & \multicolumn{4}{c}{\textbf{Multi-Choice Task}} \\
% \cmidrule(lr){2-7} \cmidrule(lr){8-11}
%  & \textbf{EE} & \textbf{POV} & \textbf{EOV} & \textbf{SE} & \textbf{EIV} & \textbf{PIV} 
%  & \textbf{POV} & \textbf{EOV} & \textbf{SE} & \textbf{MIV} \\
% \midrule
% InternVL2.5-78B & 0.7717 & 0.9784 & 0.9509 & 0.925 & 0.8770 & 0.8813 & 0.9051 & 0.9057 & 0.8631 & 0.7464 \\
% LLaVA-Video-72B & 0.8794 & 0.8721 & 0.8067 & 0.795 & 0.6475 & 0.6525 & 0.8775 & 0.9057 & 0.8460 & 0.6892 \\
% Qwen2VL-72B & 0.5506 & 0.9632 & 0.9811 & 0.9408 & 0.9180 & 0.8814 & 0.7818 & 0.7906 & 0.8160 & 0.5678 \\
% LLaVA-OneVision-72B & 0.9469 & 0.7372 & 0.6357 & 0.6081 & 0.5 & 0.3983 & 0.7836 & 0.7773 & 0.7698 & 0.5892 \\
% LLaVA-Video-7B & 0.8286 & 0.8910 & 0.8528 & 0.7814 & 0.5424 & 0.5378 & 0.9059 & 0.8976 & 0.8368 & 0.6500 \\
% Qwen2VL-7B & 0.7869 & 0.8983 & 0.7949 & 0.7713 & 0.5574 & 0.5785 & 0.7183 & 0.7288 & 0.7604 & 0.4785 \\
% Qwen2VL-2B & 0.4754 & 0.9737 & 0.9354 & 0.9308 & 0.8606 & 0.7542 & 0.6586 & 0.7436 & 0.7644 & 0.4321 \\
% LLaVA-OneVision-7B & 0.8557 & 0.8900 & 0.7763 & 0.6943 & 0.4492 & 0.3529 & 0.8369 & 0.8356 & 0.7944 & 0.5000 \\
% Aria-23B & 0.6704 & 0.9178 & 0.9463 & 0.8900 & 0.8115 & 0.7203 & 0.6894 & 0.7102 & 0.7872 & 0.5214 \\
% VILA1.5-8B & 0.8219 & 0.7101 & 0.8206 & 0.6983 & 0.4016 & 0.3729 & 0.7968 & 0.7728 & 0.7293 & 0.4678 \\
% VideoXL-7B & 0.5497 & 0.8041 & 0.8263 & 0.7973 & 0.7107 & 0.6779 & 0.6303 & 0.6932 & 0.6395 & 0.4229 \\
% LLaVA-NeXT-Video-32B & 0.8617 & 0.7600 & 0.7463 & 0.7225 & 0.6393 & 0.5593 & 0.8025 & 0.8615 & 0.7844 & 0.5964 \\
% LLaVA-NeXT-Video-7B & 0.2158 & 0.9733 & 0.9784 & 0.9700 & 0.9180 & 0.9492 & 0.5173 & 0.6674 & 0.6446 & 0.4000 \\
% LongVILA-8B & 0.9453 & 0.3302 & 0.5517 & 0.3250 & 0.1311 & 0.1780 & 0.6579 & 0.6608 & 0.6455 & 0.4714 \\
% Oryx1.5-32B & 0.2460 & 0.9448 & 0.9759 & 0.9308 & 0.9098 & 0.9322 & 0.5175 & 0.4912 & 0.5451 & 0.3285 \\
% Oryx-7B & 0.2440 & 0.9458 & 0.9713 & 0.9317 & 0.9508 & 0.9322 & 0.5020 & 0.5023 & 0.5292 & 0.3285 \\
% Oryx1.5-7B & 0.2612 & 0.9559 & 0.9370 & 0.9258 & 0.9590 & 0.8898 & 0.5566 & 0.5056 & 0.5223 & 0.3535 \\
% VideoLLaMA2.1-7B-16f & 0.3850 & 0.9563 & 0.9634 & 0.9558 & 0.8525 & 0.7712 & 0.6523 & 0.7547 & 0.7587 & 0.3857 \\
% LLaMA-VID-7B & 0.9759 & 0.0672 & 0.0322 & 0.0492 & 0.0492 & 0.0424 & 0.3132 & 0.4039 & 0.4009 & 0.2437 \\
% LLaMA-VID-Long-Video-7B & 0.7471 & 0.3291 & 0.3369 & 0.3008 & 0.2049 & 0.2796 & 0.2663 & 0.2591 & 0.2671 & 0.1964 \\
% LLaMA-VID-13B & 0.5918 & 0.7305 & 0.7192 & 0.6616 & 0.5655 & 0.4915 & 0.3573 & 0.4500 & 0.4419 & 0.2535 \\
% Video-LLaVA-7B & 0.9911 & 0.0164 & 0.0236 & 0.0150 & 0.0081 & 0.0169 & 0.2695 & 0.2813 & 0.2865 & 0.2178 \\
% \bottomrule
% \end{tabular}
% \end{table*}
%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table*}[h]
% \centering
% \scriptsize
% \caption{LVMs' performances on Stage Hallucination (Action) for Binary/Multi-Choice tasks.}
% \label{tb:ordered_event_hallucination}
% \begin{tabular}{lcccccccccccc}
% \toprule
% \textbf{Model} & \multicolumn{6}{c}{\textbf{Binary Task}} & \multicolumn{4}{c}{\textbf{Multi-Choice Task}} \\
% \cmidrule(lr){2-7} \cmidrule(lr){8-11}
%  & \textbf{EA} & \textbf{COV} & \textbf{AOV} & \textbf{SA} & \textbf{AIV} & \textbf{CIV} 
%  & \textbf{COV} & \textbf{AOV} & \textbf{SA} & \textbf{MIV} \\
% \midrule
% LLaVA-NeXT-Video-32B & 0.8617 & 0.7600 & 0.7463 & 0.7225 & 0.6393 & 0.5593 & 0.8025 & 0.8615 & 0.7844 & 0.5964 \\
% Oryx-7B & 0.2440 & 0.9458 & 0.9713 & 0.9317 & 0.9508 & 0.9322 & 0.5020 & 0.5023 & 0.5292 & 0.3285 \\
% Oryx1.5-7B & 0.2612 & 0.9559 & 0.9370 & 0.9258 & 0.9590 & 0.8898 & 0.5566 & 0.5056 & 0.5223 & 0.3535 \\
% Qwen2VL-72B & 0.5506 & 0.9632 & 0.9811 & 0.9408 & 0.9180 & 0.8814 & 0.7818 & 0.7906 & 0.8160 & 0.5678 \\
% VideoLLaMA2.1-7B-16f & 0.3850 & 0.9563 & 0.9634 & 0.9558 & 0.8525 & 0.7712 & 0.6523 & 0.7547 & 0.7587 & 0.3857 \\
% LLaVA-OneVision-72B & 0.9469 & 0.7372 & 0.6357 & 0.6081 & 0.5 & 0.3983 & 0.7836 & 0.7773 & 0.7698 & 0.5892 \\
% Qwen2VL-7B & 0.7869 & 0.8983 & 0.7949 & 0.7713 & 0.5574 & 0.5785 & 0.7183 & 0.7288 & 0.7604 & 0.4785 \\
% LLaVA-Video-72B & 0.8794 & 0.8721 & 0.8067 & 0.7950 & 0.6475 & 0.6525 & 0.8775 & 0.9057 & 0.8460 & 0.6892 \\
% InternVL2.5-78B & \textbf{0.7717} & \textbf{0.9784} & \textbf{0.9509} & \textbf{0.9250} & 0.8770 & 0.8813 & \textbf{0.9051} & \textbf{0.9057} & \textbf{0.8631} & \textbf{0.7464} \\
% LongVILA-8B & 0.9453 & 0.3302 & 0.5517 & 0.3250 & 0.1311 & 0.1780 & 0.6579 & 0.6608 & 0.6455 & 0.4714 \\
% VILA1.5-8B & 0.8219 & 0.7101 & 0.8206 & 0.6983 & 0.4016 & 0.3729 & 0.7968 & 0.7728 & 0.7293 & 0.4678 \\
% LLaMA-VID-Long-Video-7B & 0.7471 & 0.3291 & 0.3369 & 0.3008 & 0.2049 & 0.2796 & 0.2663 & 0.2591 & 0.2671 & 0.1964 \\
% LLaMA-VID-13B & 0.5918 & 0.7305 & 0.7192 & 0.6616 & 0.5655 & 0.4915 & 0.3573 & 0.4500 & 0.4419 & 0.2535 \\
% LLaVA-NeXT-Video-7B & 0.2158 & 0.9733 & 0.9784 & 0.9700 & 0.9180 & 0.9492 & 0.5173 & 0.6674 & 0.6446 & 0.4000 \\
% Aria-23B & 0.6704 & 0.9178 & 0.9463 & 0.8900 & 0.8115 & 0.7203 & 0.6894 & 0.7102 & 0.7872 & 0.5214 \\
% % VideoAgent & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% \bottomrule
% \end{tabular}
% \end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}
% \caption{Evaluation results on simple event hallucination questions. Meaning of the abbreviation can be found in \ref{event_abbreviation}.}
% \label{simpleQ_action_7}
% \centering
% \begin{tabular}{llcc}
% \toprule
% LVLM & \textbf{W Avg} & \textbf{JSD} \\
% \midrule
% InternVL2.5-78B & 0.85254 & 0.00005 \\
% LLaVA-Video-72B & 0.83019 & 0.00936 \\
% LLaVA-Video-7B & 0.80974 & 0.00803 \\
% LLaVA-OneVision-7B-chat & 0.78596 & 0.01446 \\
% LLaVA-OneVision-7B & 0.78495 & 0.01481 \\
% LLaVA-NeXT-Video-32B & 0.78447 & 0.01730 \\
% Qwen2VL-7B & 0.78279 & 0.00991 \\
% LLaVA-OneVision-72B & 0.77736 & 0.03623 \\
% Aria-23B & 0.77530 & 0.00026 \\
% Qwen2VL-72B & 0.74846 & 0.00415 \\
% VILA1.5-8B & 0.73806 & 0.02415 \\
% InternVL2.5-8B & 0.71039 & 0.05260 \\
% Qwen2VL-2B & 0.69379 & 0.00119 \\
% VideoXL-7B & 0.66517 & 0.00787 \\
% VideoLLaMA2.1-7B-16f & 0.65353 & 0.00311 \\
% LongVILA-8B & 0.64279 & 0.12937 \\
% LLaMA-VID-13B & 0.62602 & 0.02439 \\
% Oryx1.5-7B & 0.59861 & 0.00414 \\
% Oryx-7B & 0.59579 & 0.00650 \\
% Oryx1.5-32B & 0.59453 & 0.00669 \\
% LLaVA-NeXT-Video-7B & 0.58980 & 0.01182 \\
% LLaMA-VID-Long-Video-7B & 0.52466 & 0.16089 \\
% LLaMA-VID-7B & 0.51225 & 0.39224 \\
% Video-LLaVA-7B & 0.50402 & 0.43679 \\
% \color{red} VideoAgent & 0.0219 & 0.9937 \\
% LLaVA-OneVision-0.5B & 0.50056 & 0.46938 \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}
% \caption{Evaluation results on multi-choice event hallucination questions (Overall metrics only).}
% \label{mc_action_overall}
% \centering
% \begin{tabular}{lcccc}
% \hline
% \textbf{LVLM} & \textbf{Accuracy} & \textbf{OB} & \textbf{COB} & \textbf{JSD} \\
% \hline
% InternVL2.5-78B & 0.85534 & 0.01309 & 0.00989 & 0.00017 \\
% LLaVA-Video-72B & 0.82966 & 0.01253 & 0.01049 & 0.00014 \\
% LLaVA-Video-7B & 0.82264 & 0.01107 & 0.00716 & 0.00013 \\
% InternVL2.5-8B & 0.76609 & 0.01530 & 0.00924 & 0.00042 \\
% LLaVA-NeXT-Video-32B & 0.76125 & 0.01691 & 0.01277 & 0.00029 \\
% LLaVA-OneVision-7B-chat & 0.74606 & 0.02528 & 0.01474 & 0.00150 \\
% LLaVA-OneVision-7B & 0.74177 & 0.02940 & 0.01701 & 0.00198 \\
% Qwen2VL-72B & 0.73912 & 0.04514 & 0.02893 & 0.00467 \\
% LLaVA-OneVision-72B & 0.73003 & 0.02153 & 0.01364 & 0.00055 \\
% VILA1.5-8B & 0.69174 & 0.02914 & 0.01625 & 0.00180 \\
% Aria-23B & 0.67730 & 0.02706 & 0.01794 & 0.00152 \\
% Qwen2VL-7B & 0.67171 & 0.06840 & 0.04717 & 0.01047 \\
% Qwen2VL-2B & 0.64973 & 0.07865 & 0.05239 & 0.01380 \\
% VideoLLaMA2.1-7B & 0.63791 & 0.05798 & 0.02626 & 0.00588 \\
% LongVILA-8B & 0.60895 & 0.11411 & 0.08391 & 0.03425 \\
% VideoXL-7B & 0.59611 & 0.04204 & 0.02596 & 0.00335 \\
% LLaVA-NeXT-Video-7B & 0.55734 & 0.06321 & 0.03847 & 0.00891 \\
% LLaVA-OneVision-0.5B & 0.49069 & 0.11133 & 0.07676 & 0.02462 \\
% Oryx1.5-32B & 0.47065 & 0.05783 & 0.03068 & 0.00655 \\
% Oryx-7B & 0.46555 & 0.03317 & 0.01657 & 0.00230 \\
% Oryx1.5-7B & 0.48457 & 0.05427 & 0.03274 & 0.00601 \\
% VideoAgent & 0.40169 & 0.04951 & 0.05376 & 0.00409 \\
% LLaMA-VID-13B & 0.37579 & 0.13043 & 0.08911 & 0.03114 \\
% LLaMA-VID-7B & 0.34046 & 0.27100 & 0.19869 & 0.11762 \\
% \hline
% \end{tabular}
% \end{table}

% \begin{table*}
% \caption{Evaluation results on event hallucination questions (simple and multi-choice).}
% \label{combined_action}
% \centering
% \begin{tabular}{lccc}
% \hline
% \textbf{LVLM} & \textbf{W Avg} & \textbf{JSD (simple)} & \textbf{JSD (multi-choice)} \\
% \hline
% InternVL2.5-78B & 0.85254 & 0.00005 & 0.00017 \\
% LLaVA-Video-72B & 0.83019 & 0.00936 & 0.00014 \\
% LLaVA-Video-7B & 0.80974 & 0.00803 & 0.00013 \\
% LLaVA-OneVision-7B-chat & 0.78596 & 0.01446 & 0.00150 \\
% LLaVA-OneVision-7B & 0.78495 & 0.01481 & 0.00198 \\
% LLaVA-NeXT-Video-32B & 0.78447 & 0.01730 & 0.00029 \\
% Qwen2VL-7B & 0.78279 & 0.00991 & 0.00467 \\
% LLaVA-OneVision-72B & 0.77736 & 0.03623 & 0.00055 \\
% Aria-23B & 0.77530 & 0.00026 & 0.00152 \\
% Qwen2VL-72B & 0.74846 & 0.00415 & 0.00467 \\
% VILA1.5-8B & 0.73806 & 0.02415 & 0.00180 \\
% InternVL2.5-8B & 0.71039 & 0.05260 & 0.00042 \\
% Qwen2VL-2B & 0.69379 & 0.00119 & 0.01380 \\
% VideoXL-7B & 0.66517 & 0.00787 & 0.00335 \\
% VideoLLaMA2.1-7B-16f & 0.65353 & 0.00311 & 0.00588 \\
% LongVILA-8B & 0.64279 & 0.12937 & 0.03425 \\
% LLaMA-VID-13B & 0.62602 & 0.02439 & 0.03114 \\
% Oryx1.5-7B & 0.59861 & 0.00414 & 0.00601 \\
% Oryx-7B & 0.59579 & 0.00650 & 0.00230 \\
% Oryx1.5-32B & 0.59453 & 0.00669 & 0.00655 \\
% LLaVA-NeXT-Video-7B & 0.58980 & 0.01182 & 0.00891 \\
% LLaMA-VID-Long-Video-7B & 0.52466 & 0.16089 & 0.11762 \\
% LLaMA-VID-7B & 0.51225 & 0.39224 & 0.11762 \\
% Video-LLaVA-7B & 0.50402 & 0.43679 & 0.43679 \\
% \textcolor{red}{VideoAgent} & 0.0219 & 0.9937 & 0.00409 \\
% LLaVA-OneVision-0.5B & 0.50056 & 0.46938 & 0.02462 \\
% \hline
% \end{tabular}
% \end{table*}

% \begin{table}
% \caption{Evaluation results on event hallucination questions (simple and multi-choice).}
% \label{combined_action}
% \centering
% \begin{tabular}{|l|c|c|c|c|c|c|c|}
% \hline
% \textbf{LVLM} & \textbf{W Avg} & \textbf{JSD (simple)} & \textbf{Accuracy} & \textbf{OB} & \textbf{COB} & \textbf{JSD (multi-choice)} \\
% \hline
% InternVL2.5-78B & 0.85254 & 0.00005 & 0.85534 & 0.01309 & 0.00989 & 0.00017 \\
% LLaVA-Video-72B & 0.83019 & 0.00936 & 0.82966 & 0.01253 & 0.01049 & 0.00014 \\
% LLaVA-Video-7B & 0.80974 & 0.00803 & 0.82264 & 0.01107 & 0.00716 & 0.00013 \\
% LLaVA-OneVision-7B-chat & 0.78596 & 0.01446 & 0.74606 & 0.02528 & 0.01474 & 0.00150 \\
% LLaVA-OneVision-7B & 0.78495 & 0.01481 & 0.74177 & 0.02940 & 0.01701 & 0.00198 \\
% LLaVA-NeXT-Video-32B & 0.78447 & 0.01730 & 0.76125 & 0.01691 & 0.01277 & 0.00029 \\
% Qwen2VL-7B & 0.78279 & 0.00991 & 0.73912 & 0.04514 & 0.02893 & 0.00467 \\
% LLaVA-OneVision-72B & 0.77736 & 0.03623 & 0.73003 & 0.02153 & 0.01364 & 0.00055 \\
% Aria-23B & 0.77530 & 0.00026 & 0.67730 & 0.02706 & 0.01794 & 0.00152 \\
% Qwen2VL-72B & 0.74846 & 0.00415 & 0.73912 & 0.04514 & 0.02893 & 0.00467 \\
% VILA1.5-8B & 0.73806 & 0.02415 & 0.69174 & 0.02914 & 0.01625 & 0.00180 \\
% InternVL2.5-8B & 0.71039 & 0.05260 & 0.76609 & 0.01530 & 0.00924 & 0.00042 \\
% Qwen2VL-2B & 0.69379 & 0.00119 & 0.64973 & 0.07865 & 0.05239 & 0.01380 \\
% VideoXL-7B & 0.66517 & 0.00787 & 0.59611 & 0.04204 & 0.02596 & 0.00335 \\
% VideoLLaMA2.1-7B-16f & 0.65353 & 0.00311 & 0.63791 & 0.05798 & 0.02626 & 0.00588 \\
% LongVILA-8B & 0.64279 & 0.12937 & 0.60895 & 0.11411 & 0.08391 & 0.03425 \\
% LLaMA-VID-13B & 0.62602 & 0.02439 & 0.37579 & 0.13043 & 0.08911 & 0.03114 \\
% Oryx1.5-7B & 0.59861 & 0.00414 & 0.48457 & 0.05427 & 0.03274 & 0.00601 \\
% Oryx-7B & 0.59579 & 0.00650 & 0.46555 & 0.03317 & 0.01657 & 0.00230 \\
% Oryx1.5-32B & 0.59453 & 0.00669 & 0.47065 & 0.05783 & 0.03068 & 0.00655 \\
% LLaVA-NeXT-Video-7B & 0.58980 & 0.01182 & 0.55734 & 0.06321 & 0.03847 & 0.00891 \\
% LLaMA-VID-Long-Video-7B & 0.52466 & 0.16089 & 0.51225 & 0.27100 & 0.19869 & 0.11762 \\
% LLaMA-VID-7B & 0.51225 & 0.39224 & 0.34046 & 0.27100 & 0.19869 & 0.11762 \\
% Video-LLaVA-7B & 0.50402 & 0.43679 & 0.50402 & 0.43679 & 0.43679 & 0.43679 \\
% \textcolor{red}{VideoAgent} & 0.0219 & 0.9937 & 0.40169 & 0.04951 & 0.05376 & 0.00409 \\
% LLaVA-OneVision-0.5B & 0.50056 & 0.46938 & 0.49069 & 0.11133 & 0.07676 & 0.02462 \\
% \hline
% \end{tabular}
% \end{table}

% \begin{table}
% \caption{Evaluation results on event hallucination questions (simple and multi-choice).}
% \scriptsize
% \label{combined_action}
% \centering
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Model} & \multicolumn{2}{c}{\textbf{Binary Task}} & \multicolumn{2}{c}{\textbf{Multi-Choice Task}} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5}
%               & \textbf{Acc.} & \textbf{JSD.} & \textbf{Acc.} & \textbf{JSD.} \\\midrule
% % \hline
% % \textbf{LVLM} & \textbf{W Avg} & \textbf{JSD (simple)} & \textbf{Accuracy} & \textbf{JSD (multi-choice)} \\
% % \hline
% InternVL2.5-78B & 0.85254 & 0.00005 & 0.85534 & 0.00017 \\
% LLaVA-Video-72B & 0.83019 & 0.00936 & 0.82966 & 0.00014 \\
% LLaVA-Video-7B & 0.80974 & 0.00803 & 0.82264 & 0.00013 \\
% LLaVA-OneVision-7B-chat & 0.78596 & 0.01446 & 0.74606 & 0.00150 \\
% LLaVA-OneVision-7B & 0.78495 & 0.01481 & 0.74177 & 0.00198 \\
% LLaVA-NeXT-Video-32B & 0.78447 & 0.01730 & 0.76125 & 0.00029 \\
% Qwen2VL-7B & 0.78279 & 0.00991 & 0.73912 & 0.00467 \\
% LLaVA-OneVision-72B & 0.77736 & 0.03623 & 0.73003 & 0.00055 \\
% Aria-23B & 0.77530 & 0.00026 & 0.67730 & 0.00152 \\
% Qwen2VL-72B & 0.74846 & 0.00415 & 0.73912 & 0.00467 \\
% VILA1.5-8B & 0.73806 & 0.02415 & 0.69174 & 0.00180 \\
% InternVL2.5-8B & 0.71039 & 0.05260 & 0.76609 & 0.00042 \\
% Qwen2VL-2B & 0.69379 & 0.00119 & 0.64973 & 0.01380 \\
% VideoXL-7B & 0.66517 & 0.00787 & 0.59611 & 0.00335 \\
% VideoLLaMA2.1-7B-16f & 0.65353 & 0.00311 & 0.63791 & 0.00588 \\
% LongVILA-8B & 0.64279 & 0.12937 & 0.60895 & 0.03425 \\
% LLaMA-VID-13B & 0.62602 & 0.02439 & 0.37579 & 0.03114 \\
% Oryx1.5-7B & 0.59861 & 0.00414 & 0.48457 & 0.00601 \\
% Oryx-7B & 0.59579 & 0.00650 & 0.46555 & 0.00230 \\
% Oryx1.5-32B & 0.59453 & 0.00669 & 0.47065 & 0.00655 \\
% LLaVA-NeXT-Video-7B & 0.58980 & 0.01182 & 0.55734 & 0.00891 \\
% LLaMA-VID-Long-Video-7B & 0.52466 & 0.16089 & 0.51225 & 0.11762 \\
% LLaMA-VID-7B & 0.51225 & 0.39224 & 0.34046 & 0.11762 \\
% Video-LLaVA-7B & 0.50402 & 0.43679 & 0.50402 & 0.43679 \\
% \textcolor{red}{VideoAgent} & 0.0219 & 0.9937 & 0.40169 & 0.00409 \\
% LLaVA-OneVision-0.5B & 0.50056 & 0.46938 & 0.49069 & 0.02462 \\
% \hline
% \end{tabular}
% \end{table}

% \begin{table}
% \caption{LVMs' on Stage Hallucination (Action) for Binary/MC tasks}
% \label{tb:ordered_event_hallucination}
% \scriptsize
% \centering
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Model} & \multicolumn{2}{c}{\textbf{Binary Task}} & \multicolumn{2}{c}{\textbf{Multi-Choice Task}} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5}
%               & \textbf{Acc.} & \textbf{JSD.} & \textbf{Acc.} & \textbf{JSD.} \\\midrule
% LLaVA-Video-72B & 0.83019 & 0.00936 & 0.82966 & 0.00014 \\
% InternVL2.5-78B & 0.85254 & 0.00005 & 0.85534 & 0.00017 \\
% LLaVA-Video-7B & 0.80974 & 0.00803 & 0.82264 & 0.00013 \\
% LLaVA-OneVision-7B-chat & 0.78596 & 0.01446 & 0.74606 & 0.00150 \\
% LLaVA-OneVision-7B & 0.78495 & 0.01481 & 0.74177 & 0.00198 \\
% LLaVA-NeXT-Video-32B & 0.78447 & 0.01730 & 0.76125 & 0.00029 \\
% Qwen2VL-72B & 0.74846 & 0.00415 & 0.73912 & 0.00467 \\
% Aria-23B & 0.77530 & 0.00026 & 0.67730 & 0.00152 \\
% LLaVA-OneVision-72B & 0.77736 & 0.03623 & 0.73003 & 0.00055 \\
% Qwen2VL-7B & 0.78279 & 0.00991 & 0.73912 & 0.00467 \\
% VILA1.5-8B & 0.73806 & 0.02415 & 0.69174 & 0.00180 \\
% InternVL2.5-8B & 0.71039 & 0.05260 & 0.76609 & 0.00042 \\
% Qwen2VL-2B & 0.69379 & 0.00119 & 0.64973 & 0.01380 \\
% VideoXL-7B & 0.66517 & 0.00787 & 0.59611 & 0.00335 \\
% VideoLLaMA2.1-7B-16f & 0.65353 & 0.00311 & 0.63791 & 0.00588 \\
% LongVILA-8B & 0.64279 & 0.12937 & 0.60895 & 0.03425 \\
% LLaMA-VID-13B & 0.62602 & 0.02439 & 0.37579 & 0.03114 \\
% Oryx1.5-7B & 0.59861 & 0.00414 & 0.48457 & 0.00601 \\
% Oryx-7B & 0.59579 & 0.00650 & 0.46555 & 0.00230 \\
% Oryx1.5-32B & 0.59453 & 0.00669 & 0.47065 & 0.00655 \\
% LLaVA-NeXT-Video-7B & 0.58980 & 0.01182 & 0.55734 & 0.00891 \\
% % LLaMA-VID-Long-Video-7B & 0.52466 & 0.16089 & 0.51225 & 0.11762 \\
% % LLaMA-VID-7B & 0.51225 & 0.39224 & 0.34046 & 0.11762 \\
% % Video-LLaVA-7B & 0.50402 & 0.43679 & 0.50402 & 0.43679 \\
% \textcolor{red}{VideoAgent} & 0.0219 & 0.9937 & 0.40169 & 0.00409 \\
% LLaVA-OneVision-0.5B & 0.50056 & 0.46938 & 0.49069 & 0.02462 \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}
% \caption{LVMs' on Stage Hallucination (Action) for Binary/MC tasks}
% \label{tb:ordered_event_hallucination}
% \scriptsize
% % \label{combined_action}
% \centering
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Model} & \multicolumn{2}{c}{\textbf{Binary Task}} & \multicolumn{2}{c}{\textbf{Multi-Choice Task}} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5}
%               & \textbf{Acc.} & \textbf{JSD.} & \textbf{Acc.} & \textbf{JSD.} \\\midrule
% LLaVA-NeXT-Video-32B & 0.78447 & 0.01730 & 0.76125 & 0.00029 \\
% Oryx-7B & 0.59579 & 0.00650 & 0.46555 & 0.00230 \\
% Oryx1.5-7B & 0.59861 & 0.00414 & 0.48457 & 0.00601 \\
% Qwen2VL-72B & 0.74846 & 0.00415 & 0.73912 & 0.00467 \\
% VideoLLaMA2.1-7B-16f & 0.65353 & 0.00311 & 0.63791 & 0.00588 \\
% LLaVA-OneVision-72B & 0.77736 & 0.03623 & 0.73003 & 0.00055 \\
% InternVL2.5-78B & 0.85254 & 0.00005 & 0.85534 & 0.00017 \\
% LongVILA-8B & 0.64279 & 0.12937 & 0.60895 & 0.03425 \\
% VILA1.5-8B & 0.73806 & 0.02415 & 0.69174 & 0.00180 \\
% LLaMA-VID-13B & 0.62602 & 0.02439 & 0.37579 & 0.03114 \\
% LLaVA-OneVision-7B-chat & 0.78596 & 0.01446 & 0.74606 & 0.00150 \\
% LLaVA-OneVision-7B & 0.78495 & 0.01481 & 0.74177 & 0.00198 \\
% Qwen2VL-7B & 0.78279 & 0.00991 & 0.73912 & 0.00467 \\
% LLaVA-Video-72B & 0.83019 & 0.00936 & 0.82966 & 0.00014 \\
% Aria-23B & 0.77530 & 0.00026 & 0.67730 & 0.00152 \\
% Qwen2VL-2B & 0.69379 & 0.00119 & 0.64973 & 0.01380 \\
% InternVL2.5-8B & 0.71039 & 0.05260 & 0.76609 & 0.00042 \\
% VideoXL-7B & 0.66517 & 0.00787 & 0.59611 & 0.00335 \\
% LLaVA-Video-7B & 0.80974 & 0.00803 & 0.82264 & 0.00013 \\
% LLaVA-OneVision-0.5B & 0.50056 & 0.46938 & 0.49069 & 0.02462 \\
% % LLaMA-VID-Long-Video-7B & 0.52466 & 0.16089 & 0.51225 & 0.11762 \\
% % LLaMA-VID-7B & 0.51225 & 0.39224 & 0.34046 & 0.11762 \\
% % Video-LLaVA-7B & 0.50402 & 0.43679 & 0.50402 & 0.43679 \\
% \textcolor{red}{VideoAgent} & 0.0219 & 0.9937 & 0.40169 & 0.00409 \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}
% \caption{LVMs' on Stage: Non-dialogue for Binary/MC tasks}
% \label{tb:ordered_event_hallucination}
% \scriptsize
% % \label{combined_action}
% \centering
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Model} & \multicolumn{2}{c}{\textbf{Binary Task}} & \multicolumn{2}{c}{\textbf{MC Task}} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5}
%               & \textbf{Acc.} & \textbf{JSD.} & \textbf{Acc.} & \textbf{JSD.} \\\midrule
% LLaVA-NeXT-Video-32B\textsuperscript{\(\star\)} & 0.78447 & 0.01730 & 0.76125 & 0.00029 \\
% Oryx-7B\textsuperscript{\(\ddagger\)} & 0.59579 & 0.00650 & 0.46555 & 0.00230 \\
% Oryx1.5-7B\textsuperscript{\(\ddagger\)} & 0.59861 & 0.00414 & 0.48457 & 0.00601 \\
% Oryx1.5-32B\textsuperscript{\(\ddagger\)}     & 0.59453 & 0.00669 & 0.47065 & 0.00655\\
% Qwen2VL-72B\textsuperscript{\(\ddagger\)} & 0.74846 & 0.00415 & 0.73912 & 0.00467 \\
% VideoLLaMA2.1-7B-16f\textsuperscript{\(\ddagger\)} & 0.65353 & 0.00311 & 0.63791 & 0.00588 \\
% LLaVA-OneVision-72B\textsuperscript{\(\ddagger\)} & 0.77736 & 0.03623 & 0.73003 & 0.00055 \\
% LLaVA-Video-72B\textsuperscript{\(\ddagger\)} & 0.83019 & 0.00936 & 0.82966 & 0.00014 \\
% InternVL2.5-78B\textsuperscript{\(\mathsection\)} & \textbf{0.85254} & 0.00005 & \textbf{0.85534} & 0.00017 \\
% LongVILA-8B\textsuperscript{\(\sharp\)} & 0.64279 & 0.12937 & 0.60895 & 0.03425 \\
% VILA1.5-8B\textsuperscript{\(\sharp\)} & 0.73806 & 0.02415 & 0.69174 & 0.00180 \\
% LLaMA-VID-Long-Video-7B\textsuperscript{\(\star\)} & 0.52466 & 0.16089 & 0.24726 & 0.19453 \\
% LLaMA-VID-13B\textsuperscript{\(\star\)} & 0.62602 & 0.02439 & 0.37579 & 0.03114 \\
% LLaVA-NeXT-Video-7B\textsuperscript{\(\star\)} & 0.58980 & 0.01182 & 0.55734 & 0.00891 \\
% Aria-23B\textsuperscript{\(\pounds\)} & 0.77530 & 0.00026 & 0.67730 & 0.00152 \\
% VideoAgent\textsuperscript{\(\natural\)} & 0.58139 & 0.00056 & 0.40169 & 0.00409 \\
% \hline
% \end{tabular}
% \end{table}

% \begin{table}
% \caption{LVMs' on Stage: Non-dialogue for Binary/MC tasks}
% \label{tb:ordered_event_hallucination}
% \scriptsize
% \centering
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Model} & \multicolumn{2}{c}{\textbf{Binary Task (\%)}} & \multicolumn{2}{c}{\textbf{MC Task (\%)}} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5}
%               & \textbf{Acc.} & \textbf{JSD-b.} & \textbf{Acc.} & \textbf{JSD-m.} \\\midrule
% LLaVA-NeXT-Video-32B\textsuperscript{\(\star\)} & 78.4 & 1.73 & 76.1 & 0.03 \\
% Oryx-7B\textsuperscript{\(\ddagger\)} & 59.6 & 0.65 & 46.6 & 0.23 \\
% Oryx1.5-7B\textsuperscript{\(\ddagger\)} & 59.9 & 0.41 & 48.5 & 0.60 \\
% Oryx1.5-32B\textsuperscript{\(\ddagger\)}     & 59.5 & 0.67 & 47.1 & 0.66 \\
% Qwen2VL-72B\textsuperscript{\(\ddagger\)} & 74.8 & 0.42 & 73.9 & 0.47 \\
% VideoLLaMA2.1-7B-16f\textsuperscript{\(\ddagger\)} & 65.4 & 0.31 & 63.8 & 0.59 \\
% LLaVA-OneVision-72B\textsuperscript{\(\ddagger\)} & 77.7 & 3.62 & 73.0 & 0.06 \\
% LLaVA-Video-72B\textsuperscript{\(\ddagger\)} & 83.0 & 0.94 & 83.0 & 0.01 \\
% InternVL2.5-78B\textsuperscript{\(\mathsection\)} & \textbf{85.3} & 0.01 & \textbf{85.5} & 0.02 \\
% LongVILA-8B\textsuperscript{\(\sharp\)} & 64.3 & 12.9 & 60.9 & 3.43 \\
% VILA1.5-8B\textsuperscript{\(\sharp\)} & 73.8 & 2.42 & 69.2 & 0.18 \\
% LLaMA-VID-Long-Video-7B\textsuperscript{\(\star\)} & 52.5 & 16.1 & 24.7 & 19.5 \\
% LLaMA-VID-13B\textsuperscript{\(\star\)} & 62.6 & 2.44 & 37.6 & 3.11 \\
% LLaVA-NeXT-Video-7B\textsuperscript{\(\star\)} & 58.9 & 1.18 & 55.7 & 0.89 \\
% Aria-23B\textsuperscript{\(\pounds\)} & 77.5 & 0.03 & 67.7 & 0.15 \\
% VideoAgent\textsuperscript{\(\natural\)} & 58.1 & 0.06 & 40.2 & 0.41 \\
% \hline
% \end{tabular}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
    \vspace{-0.3cm}
    \centering
    \label{fig:ordered_event_hallucination}
    \includegraphics[width=\columnwidth]{fig/action_result.pdf}
    \vspace{-0.8cm}
    \Description{action_result}
    \caption{Non-dialogue Hallucination for Binary/MC tasks}
    \vspace{-0.4cm}
\end{figure}
% \begin{table}
% \centering
% \caption{LVMs' on Stage: Non-dialogue for Binary/MC tasks}
% \label{tb:ordered_event_hallucination}
% % \small
% % \footnotesize
% % \scriptsize
% \centering
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Model} & \multicolumn{2}{c}{\textbf{Binary \%}} & \multicolumn{2}{c}{\textbf{MC \%}} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5}
%               & Acc & JSD & Acc & JSD \\\midrule
% LLaVA-NV-32B\textsuperscript{\(\star\)} & 78.4 & 8.01 & 76.1 & 0.08 \\
% Oryx-7B\textsuperscript{\(\ddagger\)} & 59.6 & 3.01 & 46.6 & 0.61 \\
% Oryx1.5-7B\textsuperscript{\(\ddagger\)} & 59.9 & 1.90 & 48.5 & 1.58 \\
% Oryx1.5-32B\textsuperscript{\(\ddagger\)}     & 59.5 & 3.10 & 47.1 & 1.74 \\
% Qwen2VL-72B\textsuperscript{\(\ddagger\)} & 74.8 & 1.94 & 73.9 & 1.24 \\
% VideoLLaMA2.1-7B\textsuperscript{\(\ddagger\)} & 65.4 & 1.44 & 63.8 & 1.55 \\
% LLaVA-OV-72B\textsuperscript{\(\ddagger\)} & 77.7 & 16.8 & 73.0 & 0.16 \\
% LLaVA-Video-72B\textsuperscript{\(\ddagger\)} & 83.0 & 4.35 & 83.0 & 0.03 \\
% InternVL2.5-78B\textsuperscript{\(\mathsection\)} & \textbf{85.3} & 0.05 & \textbf{85.5} & 0.05 \\
% LongVILA-8B\textsuperscript{\(\sharp\)} & 64.3 & 59.7 & 60.9 & 9.03 \\
% VILA1.5-8B\textsuperscript{\(\sharp\)} & 73.8 & 11.2 & 69.2 & 0.47 \\
% LLaMA-VID-LV-7B\textsuperscript{\(\star\)} & 52.5 & 74.5 & 24.7 & 51.3 \\
% LLaMA-VID-13B\textsuperscript{\(\star\)} & 62.6 & 11.3 & 37.6 & 8.21 \\
% LLaVA-NV-7B\textsuperscript{\(\star\)} & 58.9 & 5.46 & 55.7 & 2.34 \\
% Aria-23B\textsuperscript{\(\pounds\)} & 77.5 & 0.14 & 67.7 & 0.40 \\
% VideoAgent\textsuperscript{\(\natural\)} & 58.1 & 0.28 & 40.2 & 1.08 \\
% \hline
% GPT-4o & 81.4 & 0.15 & 67.3 & 0.66\\
% \bottomrule
% \end{tabular}
% \vspace{-0.7cm}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vspace{-0.2cm}
% Qwen2VL-7B\textsuperscript{\(\ddagger\)} & 0.78279 & 0.00991 & 0.73912 & 0.00467 \\
% LLaVA-OneVision-7B-chat & 0.78596 & 0.01446 & 0.74606 & 0.00150 \\
% LLaVA-OneVision-7B & 0.78495 & 0.01481 & 0.74177 & 0.00198 \\
% Qwen2VL-2B & 0.69379 & 0.00119 & 0.64973 & 0.01380 \\
% VideoXL-7B & 0.66517 & 0.00787 & 0.59611 & 0.00335 \\
% LLaMA-VID-7B & 0.51225 & 0.39224 & 0.34046 & 0.11762 \\
% Video-LLaVA-7B & 0.50402 & 0.43679 & 0.50402 & 0.43679 \\
% LLaVA-OneVision-0.5B & 0.50056 & 0.46938 & 0.49069 & 0.02462 \\




% \begin{table*}[h]
% \centering
% \scriptsize
% \caption{LVMs' performances on Stage Hallucination (Talking) for Binary/Multi-Choice tasks.}
% \label{combined_talk_event}
% \begin{tabular}{lcccccccc}
% \toprule
% \textbf{LVLM} & \multicolumn{4}{c}{\textbf{Simple Task}} & \multicolumn{2}{c}{\textbf{Multi-Choice Task}} \\
% \cmidrule(lr){2-5} \cmidrule(lr){6-7}
%  & \textbf{EE} & \textbf{POV} & \textbf{EOV} & \textbf{PIV} & \textbf{POV} & \textbf{PIV} \\
% \midrule
% InternVL2.5-78B & 0.7216 & 0.9859 & 0.9539 & 0.6365 & 0.9488 & 0.7275 \\
% LLaVA-Video-72B & 0.8814 & 0.9186 & 0.8526 & 0.4200 & 0.9235 & 0.7198 \\
% Qwen2VL-72B & 0.5779 & 0.9859 & 0.9653 & 0.7255 & 0.9114 & 0.6762 \\
% LLaVA-OneVision-72B & 0.9227 & 0.8062 & 0.7202 & 0.3337 & 0.8835 & 0.6867 \\
% LLaVA-Video-7B & 0.8333 & 0.9454 & 0.8673 & 0.4924 & 0.9312 & 0.7077 \\
% Qwen2VL-7B & 0.7994 & 0.9454 & 0.8069 & 0.5545 & 0.8513 & 0.6428 \\
% Qwen2VL-2B & 0.6873 & 0.9723 & 0.9100 & 0.6289 & 0.8362 & 0.6183 \\
% LLaVA-OneVision-7B & 0.8784 & 0.9165 & 0.7855 & 0.3648 & 0.8951 & 0.6016 \\
% Aria-23B & 0.6070 & 0.9766 & 0.9479 & 0.6476 & 0.8500 & 0.6562 \\
% VILA1.5-8B & 0.8779 & 0.9023 & 0.8099 & 0.4062 & 0.8968 & 0.6794 \\
% LLaVA-NeXT-Video-32B & 0.8897 & 0.7315 & 0.8463 & 0.2800 & 0.8590 & 0.6433 \\
% Oryx1.5-32B & 0.6122 & 0.9752 & 0.8939 & 0.7758 & 0.8530 & 0.6390 \\
% Oryx1.5-7B & 0.6191 & 0.9524 & 0.8916 & 0.7351 & 0.8345 & 0.6540 \\
% Oryx-7B & 0.6187 & 0.9650 & 0.8912 & 0.7620 & 0.8302 & 0.6519 \\
% LLaVA-NeXT-Video-7B & 0.6143 & 0.9414 & 0.9522 & 0.7612 & 0.7370 & 0.5791 \\
% VideoLLaMA2.1-7B-16f & 0.4902 & 0.9779 & 0.9643 & 0.7744 & 0.8392 & 0.6415 \\
% LLaMA-VID-13B & 0.7863 & 0.7445 & 0.8800 & 0.3289 & 0.6308 & 0.4611 \\
% LLaMA-VID-7B & 0.9973 & 0.0127 & 0.0952 & 0.0034 & 0.3970 & 0.3330 \\
% LLaMA-VID-Long-Video-7B & 0.8080 & 0.1904 & 0.1790 & 0.2427 & 0.3085 & 0.3055 \\
% Video-LLaVA-7B & 1.0000 & 0.0014 & 0.0224 & 0.0000 & 0.2930 & 0.2784 \\
% \bottomrule
% \end{tabular}
% \end{table*}
%%%%%%%%%%%%%%%%%%%%%
% \begin{table*}[h]
% \centering
% \scriptsize
% \caption{LVMs' performances on Stage Hallucination (Talking) for Binary/Multi-Choice tasks.}
% \label{tb:reordered_talk_event}
% \begin{tabular}{lcccccccc}
% \toprule
% \textbf{Model} & \multicolumn{4}{c}{\textbf{Binary Task}} & \multicolumn{2}{c}{\textbf{Multi-Choice Task}} \\
% \cmidrule(lr){2-5} \cmidrule(lr){6-7}
%  & \textbf{EE} & \textbf{POV} & \textbf{EOV} & \textbf{PIV} & \textbf{POV} & \textbf{PIV} \\
% \midrule
% LLaVA-NeXT-Video-32B & 0.8897 & 0.7315 & 0.8463 & 0.2800 & 0.8590 & 0.6433 \\
% Oryx-7B & 0.6187 & 0.9650 & 0.8912 & \textbf{0.7620} & 0.8302 & 0.6519 \\
% Oryx1.5-7B & 0.6191 & 0.9524 & 0.8916 & 0.7351 & 0.8345 & 0.6540 \\
% Qwen2VL-72B & 0.5779 & \textbf{0.9859} & \textbf{0.9653} & 0.7255 & 0.9114 & 0.6762 \\
% VideoLLaMA2.1-7B-16f & 0.4902 & 0.9779 & 0.9643 & 0.7744 & 0.8392 & 0.6415 \\
% LLaVA-OneVision-72B & 0.9227 & 0.8062 & 0.7202 & 0.3337 & 0.8835 & 0.6867 \\
% Qwen2VL-7B & 0.7994 & 0.9454 & 0.8069 & 0.5545 & 0.8513 & 0.6428 \\
% LLaVA-Video-72B & 0.8814 & 0.9186 & 0.8526 & 0.4200 & 0.9235 & 0.7198 \\
% InternVL2.5-78B & 0.7216 & 0.9859 & 0.9539 & 0.6365 & \textbf{0.9488} & \textbf{0.7275} \\
% LongVILA-8B & \textbf{0.9309} & 0.6158 & 0.3025 & 0.2420 & 0.8513 & 0.6781 \\
% VILA1.5-8B & 0.8779 & 0.9023 & 0.8099 & 0.4062 & 0.8968 & 0.6794 \\
% LLaMA-VID-Long-Video-7B & 0.8080 & 0.1904 & 0.1790 & 0.2427 & 0.3085 & 0.3055 \\
% LLaMA-VID-13B & 0.7863 & 0.7445 & 0.8800 & 0.3289 & 0.6308 & 0.4611 \\
% LLaVA-NeXT-Video-7B & 0.6143 & 0.9414 & 0.9522 & 0.7612 & 0.7370 & 0.5791 \\
% Aria-23B & 0.6070 & 0.9766 & 0.9479 & 0.6476 & 0.8500 & 0.6562 \\
% \bottomrule
% \end{tabular}
% \end{table*}
%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}
%   \caption{Evaluation results on the event "talk" with simple question format. Meaning of the abbreviation can be found in \ref{event_abbreviation}.}
%   \label{simpleQ_talk}
%   \centering
%   \begin{tabular}{|l|l|l|}
%     \hline
%     \textbf{LVLM} & \textbf{Accuracy-BI} & \textbf{JSD-BI} \\
%     \hline
%     LLaVA-Video-72B & 0.80595 & 0.00951 \\
%     LLaVA-Video-7B & 0.80082 & 0.00683 \\
%     VILA1.5-8B & 0.79207 & 0.01546 \\
%     InternVL2.5-78B & 0.79024 & 0.00001 \\
%     Qwen2VL-7B & 0.78416 & 0.00837 \\
%     LLaVA-OneVision-7B-chat & 0.78519 & 0.01581 \\
%     LLaVA-OneVision-7B & 0.78369 & 0.01671 \\
%     LLaVA-OneVision-72B & 0.77140 & 0.02492 \\
%     Qwen2VL-2B & 0.76223 & 0.00095 \\
%     LLaVA-NeXT-Video-32B & 0.75449 & 0.02242 \\
%     LLaVA-NeXT-Video-7B & 0.74967 & 0.00006 \\
%     Oryx1.5-32B & 0.74696 & 0.00015 \\
%     Oryx-7B & 0.74578 & 0.00037 \\
%     Oryx1.5-7B & 0.73947 & 0.00070 \\
%     Qwen2VL-72B & 0.73510 & 0.00350 \\
%     Aria-23B & 0.73221 & 0.00001 \\
%     LLaMA-VID-13B & 0.71878 & 0.02283 \\
%     VideoXL-7B & 0.71121 & 0.01506 \\
%     VideoLLaMA2.1-7B-16f & 0.69792 & 0.00107 \\
%     InternVL2.5-8B & 0.69924 & 0.02956 \\
%     LongVILA-8B & 0.65889 & 0.12075 \\
%     LLaMA-VID-7B & 0.51728 & 0.40015 \\
%     LLaMA-VID-Long-Video-7B & 0.50609 & 0.24305 \\
%     LLaVA-OneVision-0.5B & 0.50061 & 0.47166 \\
%     Video-LLaVA-7B & 0.50400 & 0.45490 \\
%     \hline
%   \end{tabular}
% \end{table}

% \begin{table}
%   \centering
%   \begin{tabular}{|l|l|l|}
%     \hline
%     \textbf{LVLM} & \textbf{Accuracy-MC} & \textbf{JSD-MC} \\
%     \hline
%     InternVL2.5-78B & 0.83820 & 0.00034 \\
%     LLaVA-Video-72B & 0.82166 & 0.00014 \\
%     LLaVA-Video-7B & 0.81951 & 0.00012 \\
%     Qwen2VL-72B & 0.79387 & 0.00559 \\
%     VILA1.5-8B & 0.78814 & 0.00029 \\
%     LLaVA-OneVision-72B & 0.78513 & 0.00009 \\
%     InternVL2.5-8B & 0.78061 & 0.00044 \\
%     LongVILA-8B & 0.76472 & 0.00679 \\
%     Aria-23B & 0.75330 & 0.00081 \\
%     LLaVA-NeXT-Video-32B & 0.75118 & 0.00059 \\
%     LLaVA-OneVision-7B-chat & 0.75075 & 0.00059 \\
%     LLaVA-OneVision-7B & 0.74839 & 0.00058 \\
%     Qwen2VL-7B & 0.74710 & 0.00655 \\
%     Oryx1.5-32B & 0.74602 & 0.00189 \\
%     Oryx1.5-7B & 0.74431 & 0.00062 \\
%     Oryx-7B & 0.74108 & 0.00139 \\
%     VideoLLaMA2.1-7B-16f & 0.74044 & 0.00112 \\
%     Qwen2VL-2B & 0.72733 & 0.00996 \\
%     LLaVA-OneVision-0.5B & 0.72174 & 0.00454 \\
%     VideoXL-7B & 0.71612 & 0.00034 \\
%     LLaVA-NeXT-Video-7B & 0.65813 & 0.01391 \\
%     LLaMA-VID-13B & 0.54598 & 0.02018 \\
%     LLaMA-VID-7B & 0.36506 & 0.15487 \\
%     LLaMA-VID-Long-Video-7B & 0.30705 & 0.11542 \\
%     Video-LLaVA-7B & 0.28578 & 0.29504 \\
%     \hline
%   \end{tabular}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}
%   \caption{Evaluation results for the "talk" event with both simple question and multiple choice formats. The abbreviations for the metrics are defined in \ref{event_abbreviation}.}
%   \label{combined_table}
%   \centering
%   \begin{tabular}{|l|l|l|l|l|}
%     \hline
%     \textbf{LVLM} & \textbf{Accuracy-BI} & \textbf{JSD-BI} & \textbf{Accuracy-MC} & \textbf{JSD-MC} \\
%     \hline
%     LLaVA-Video-72B & 0.80595 & 0.00951 & 0.82166 & 0.00014 \\
%     LLaVA-Video-7B & 0.80082 & 0.00683 & 0.81951 & 0.00012 \\
%     VILA1.5-8B & 0.79207 & 0.01546 & 0.78814 & 0.00029 \\
%     InternVL2.5-78B & 0.79024 & 0.00001 & 0.83820 & 0.00034 \\
%     Qwen2VL-7B & 0.78416 & 0.00837 & 0.74710 & 0.00655 \\
%     LLaVA-OneVision-7B-chat & 0.78519 & 0.01581 & 0.75075 & 0.00059 \\
%     LLaVA-OneVision-7B & 0.78369 & 0.01671 & 0.74839 & 0.00058 \\
%     LLaVA-OneVision-72B & 0.77140 & 0.02492 & 0.78513 & 0.00009 \\
%     Qwen2VL-2B & 0.76223 & 0.00095 & 0.72733 & 0.00996 \\
%     LLaVA-NeXT-Video-32B & 0.75449 & 0.02242 & 0.75118 & 0.00059 \\
%     LLaVA-NeXT-Video-7B & 0.74967 & 0.00006 & 0.65813 & 0.01391 \\
%     Oryx1.5-32B & 0.74696 & 0.00015 & 0.74602 & 0.00189 \\
%     Oryx-7B & 0.74578 & 0.00037 & 0.74108 & 0.00139 \\
%     Oryx1.5-7B & 0.73947 & 0.00070 & 0.74431 & 0.00062 \\
%     Qwen2VL-72B & 0.73510 & 0.00350 & 0.79387 & 0.00559 \\
%     Aria-23B & 0.73221 & 0.00001 & 0.75330 & 0.00081 \\
%     LLaMA-VID-13B & 0.71878 & 0.02283 & 0.54598 & 0.02018 \\
%     VideoXL-7B & 0.71121 & 0.01506 & 0.71612 & 0.00034 \\
%     VideoLLaMA2.1-7B-16f & 0.69792 & 0.00107 & 0.74044 & 0.00112 \\
%     InternVL2.5-8B & 0.69924 & 0.02956 & 0.78061 & 0.00044 \\
%     LongVILA-8B & 0.65889 & 0.12075 & 0.76472 & 0.00679 \\
%     LLaMA-VID-7B & 0.51728 & 0.40015 & 0.36506 & 0.15487 \\
%     LLaMA-VID-Long-Video-7B & 0.50609 & 0.24305 & 0.30705 & 0.11542 \\
%     LLaVA-OneVision-0.5B & 0.50061 & 0.47166 & 0.72174 & 0.00454 \\
%     Video-LLaVA-7B & 0.50400 & 0.45490 & 0.28578 & 0.29504 \\
%     \hline
%   \end{tabular}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table}
% \caption{LVMs' on Stage: Dialogue for Binary/MC tasks}
% \label{tb:reordered_talk_event}
% \scriptsize
%   \centering
%   \begin{tabular}{lcccc}
% \toprule
% \textbf{Model} & \multicolumn{2}{c}{\textbf{Binary Task}} & \multicolumn{2}{c}{\textbf{Multi-Choice Task}} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5}
%               & \textbf{Acc.} & \textbf{JSD-b.} & \textbf{Acc.} & \textbf{JSD-m.} \\\midrule
%     LLaVA-NeXT-Video-32B\textsuperscript{\(\star\)} & 0.75449 & 0.02242 & 0.75118 & 0.00059 \\
%     Oryx-7B\textsuperscript{\(\ddagger\)} & 0.74578 & 0.00037 & 0.74108 & 0.00139 \\
%     Oryx1.5-7B\textsuperscript{\(\ddagger\)} & 0.73947 & 0.00070 & 0.74431 & 0.00062 \\

% Oryx1.5-32B\textsuperscript{\(\ddagger\)} & 0.74696 & 0.00015 & 0.74602 & 0.00189\\

%     Qwen2VL-72B\textsuperscript{\(\ddagger\)} & 0.73510 & 0.00350 & 0.79387 & 0.00559 \\
%     VideoLLaMA2.1-7B-16f\textsuperscript{\(\ddagger\)} & 0.69792 & 0.00107 & 0.74044 & 0.00112 \\
%     LLaVA-OneVision-72B\textsuperscript{\(\ddagger\)} & 0.77140 & 0.02492 & 0.78513 & 0.00009 \\
%     LLaVA-Video-72B\textsuperscript{\(\ddagger\)} & \textbf{0.80595} & 0.00951 & 0.82166 & 0.00014 \\
%     InternVL2.5-78B\textsuperscript{\(\mathsection\)} & 0.79024 & 0.00001 & \textbf{0.83820} & 0.00034 \\
%     LongVILA-8B\textsuperscript{\(\sharp\)} & 0.65889 & 0.12075 & 0.76472 & 0.00679 \\
%     VILA1.5-8B\textsuperscript{\(\sharp\)} & 0.79207 & 0.01546 & 0.78814 & 0.00029 \\
%     LLaMA-VID-Long-Video-7B\textsuperscript{\(\star\)} & 0.50609 & 0.24305 & 0.30705 & 0.11542 \\
%     LLaMA-VID-13B\textsuperscript{\(\star\)} & 0.71878 & 0.02283 & 0.54598 & 0.02018 \\
%     LLaVA-NeXT-Video-7B\textsuperscript{\(\star\)} & 0.74967 & 0.00006 & 0.65813 & 0.01391 \\
%     Aria-23B\textsuperscript{\(\pounds\)} & 0.73221 & 0.00001 & 0.75330 & 0.00081 \\
%     \hline
%   \end{tabular}
% \end{table}
%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%

% \begin{table}
% \caption{LVMs' on Stage: Dialogue for Binary/MC tasks}
% \label{tb:reordered_talk_event}
% % \footnotesize
%   \centering
%   \begin{tabular}{lcccc}
% \toprule
% \textbf{Model} & \multicolumn{2}{c}{\textbf{Binary \%}} & \multicolumn{2}{c}{\textbf{MC \%}} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5}
%               % & \textbf{Acc} & \textbf{Jsd} & \textbf{Acc} & \textbf{Jsd} \\\midrule
%               & Acc & JSD & Acc & JSD \\\midrule
%     LLaVA-NV-32B\textsuperscript{\(\star\)} & 75.4 & 10.4 & 75.1 & 0.16 \\
%     Oryx-7B\textsuperscript{\(\ddagger\)} & 74.6 & 0.17 & 74.1 & 0.37 \\
%     Oryx1.5-7B\textsuperscript{\(\ddagger\)} & 73.9 & 0.32 & 74.4 & 0.16 \\
%     Oryx1.5-32B\textsuperscript{\(\ddagger\)} & 74.7 & 0.07 & 74.6 & 0.50 \\
%     Qwen2VL-72B\textsuperscript{\(\ddagger\)} & 73.5 & 1.62 & 79.4 & 1.47 \\
%     VideoLLaMA2.1-7B\textsuperscript{\(\ddagger\)} & 69.8 & 0.50 & 74.0 & 0.30 \\
%     LLaVA-OV-72B\textsuperscript{\(\ddagger\)} & 77.1 & 11.5 & 78.5 & 0.02 \\
%     LLaVA-Video-72B\textsuperscript{\(\ddagger\)} & \textbf{80.6} & 4.40 & 82.2 & 0.04 \\
%     InternVL2.5-78B\textsuperscript{\(\mathsection\)} & 79.0 & 0.01 & \textbf{83.8} & 0.09 \\
%     LongVILA-8B\textsuperscript{\(\sharp\)} & 65.9 & 55.9 & 76.5 & 1.79 \\
%     VILA1.5-8B\textsuperscript{\(\sharp\)} & 79.2 & 7.16 & 78.8 & 0.08 \\
%     LLaMA-VID-LV-7B\textsuperscript{\(\star\)} & 50.6 & 100. & 30.7 & 30.4 \\
%     LLaMA-VID-13B\textsuperscript{\(\star\)} & 71.9 & 10.6 & 54.6 & 5.31 \\
%     LLaVA-NV-7B\textsuperscript{\(\star\)} & 75.0 & 0.03 & 65.8 & 3.66 \\
%     Aria-23B\textsuperscript{\(\pounds\)} & 73.2 & 0.01 & 75.3 & 0.21 \\
%     \hline
%     GPT-4o & 79.3 & 0.14 & 73.4 & 0.45\\
%     \bottomrule
%   \end{tabular}
% \vspace{-0.8cm}
% \end{table}
%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
\vspace{-0.3cm}
    \centering
    \includegraphics[width=\columnwidth]{fig/talk_result.pdf} % Adjust width to fit the entire column width
    \vspace{-0.8cm}
    \caption{Dialogue Hallucination for Binary/MC tasks}
    \label{fig:reordered_talk_event}
    % \vspace{-0.8cm}
\end{figure}
% \begin{table}
%   \caption{Evaluation results on the event "talk" with multi-choice question format. Meaning of the abbreviation can be found in \ref{event_abbreviation}.}
%   \label{mc_talk}
%   \centering
%   \begin{tabular}{|l|l|l|l|l|}
%     \hline
%     \textbf{LVLM} & \textbf{Accuracy} & \textbf{OB} & \textbf{COB} & \textbf{JSD} \\
%     \hline
%     InternVL2.5-78B & 0.83820 & 0.01543 & 0.01114 & 0.00034 \\
%     LLaVA-Video-72B & 0.82166 & 0.00290 & 0.00526 & 0.00014 \\
%     LLaVA-Video-7B & 0.81951 & 0.01033 & 0.00862 & 0.00012 \\
%     Qwen2VL-72B & 0.79387 & 0.05425 & 0.03737 & 0.00559 \\
%     VILA1.5-8B & 0.78814 & 0.01139 & 0.00895 & 0.00029 \\
%     LLaVA-OneVision-72B & 0.78513 & 0.00672 & 0.00722 & 0.00009 \\
%     InternVL2.5-8B & 0.78061 & 0.01118 & 0.00644 & 0.00044 \\
%     LongVILA-8B & 0.76472 & 0.05053 & 0.02672 & 0.00679 \\
%     Aria-23B & 0.75330 & 0.01528 & 0.00845 & 0.00081 \\
%     LLaVA-NeXT-Video-32B & 0.75118 & 0.01603 & 0.00621 & 0.00059 \\
%     LLaVA-OneVision-7B-chat & 0.75075 & 0.01435 & 0.00836 & 0.00059 \\
%     LLaVA-OneVision-7B & 0.74839 & 0.01405 & 0.00847 & 0.00058 \\
%     Qwen2VL-7B & 0.74710 & 0.05738 & 0.03913 & 0.00655 \\
%     Oryx1.5-32B & 0.74602 & 0.03544 & 0.02362 & 0.00189 \\
%     Oryx1.5-7B & 0.74431 & 0.02129 & 0.01510 & 0.00062 \\
%     Oryx-7B & 0.74108 & 0.02634 & 0.01075 & 0.00139 \\
%     VideoLLaMA2.1-7B-16f & 0.74044 & 0.02815 & 0.01748 & 0.00112 \\
%     Qwen2VL-2B & 0.72733 & 0.06667 & 0.04773 & 0.00996 \\
%     LLaVA-OneVision-0.5B & 0.72174 & 0.03995 & 0.02286 & 0.00454 \\
%     VideoXL-7B & 0.71612 & 0.01767 & 0.01489 & 0.00034 \\
%     LLaVA-NeXT-Video-7B & 0.65813 & 0.07936 & 0.03629 & 0.01391 \\
%     LLaMA-VID-13B & 0.54598 & 0.10499 & 0.05561 & 0.02018 \\
%     LLaMA-VID-7B & 0.36506 & 0.30118 & 0.21621 & 0.15487 \\
%     LLaMA-VID-Long-Video-7B & 0.30705 & 0.21638 & 0.20458 & 0.11542 \\
%     Video-LLaVA-7B & 0.28578 & 0.40171 & 0.34912 & 0.29504 \\
%     \hline
%   \end{tabular}
% \end{table}
%%%%%%%%%%%%%%%%%%%
